Dynamic size counting in population protocols

The population protocol model describes a network of anonymous agents that interact asynchronously in pairs chosen at random. Each agent starts in the same initial state $s$. We introduce the *dynamic size counting* problem: approximately counting the number of agents in the presence of an adversary who at any time can remove any number of agents or add any number of new agents in state $s$. A valid solution requires that after each addition/removal event, resulting in population size $n$, with high probability each agent "quickly" computes the same constant-factor estimate of the value $\log_2 n$ (how quickly is called the *convergence* time), which remains the output of every agent for as long as possible (the *holding* time). Since the adversary can remove agents, the holding time is necessarily finite: even after the adversary stops altering the population, it is impossible to *stabilize* to an output that never again changes. We first show that a protocol solves the dynamic size counting problem if and only if it solves the *loosely-stabilizing counting* problem: that of estimating $\log n$ in a *fixed-size* population, but where the adversary can initialize each agent in an arbitrary state, with the same convergence time and holding time. We then show a protocol solving the loosely-stabilizing counting problem with the following guarantees: if the population size is $n$, $M$ is the largest initial estimate of $\log n$, and s is the maximum integer initially stored in any field of the agents' memory, we have expected convergence time $O(\log n + \log M)$, expected polynomial holding time, and expected memory usage of $O(\log^2 (s) + (\log \log n)^2)$ bits. Interpreted as a dynamic size counting protocol, when changing from population size $n_{prev}$ to $n_{next}$, the convergence time is $O(\log n_{next} + \log \log n_{prev})$.

==> sections/sg_markov.tex <==
\subsection{$\SG$ distribution (Markov chain)}
We can analyze the distribution of $\SG$ values using the truncated Markov chain and Chernoff bound for Markov chains. 


\begin{figure}[ht!]
	\centering
	\begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth, draft=false]{figures/sg_chain}
        \caption{The infinite chain of $\SG$ values. }
        \label{fig:sg-chain-unbounded}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth, draft=false]{figures/sg_chain_truncated}
        \caption{The truncated chain that maps all the states $k+1$, $k+2$, $\ldots$ to state $k+1$. The truncated chain is also known as the ``winning streak''\cite[add citation]{?}. }
        \label{fig:sg-chain-truncated}
    \end{subfigure}
	\caption{This figure represents how the original $\SG$ chain and the truncated version that we use for analysis update.}
	\label{fig:sg-chain}
\end{figure}



\begin{lemma}\label{lem:sg-stationary}
For both truncated and non-truncated chains at the stationary distribution of $\SG$-chain: $\pi_{i} = (1/2)^i$.
\end{lemma}
\begin{proof}
(non truncated version, it is the same for the truncated chain)
Let $X_i$ be the value of $\SG$ after $i$ interactions for a fixed agent. With the definition of $\SG$ given in protocol~\ref{protocol:stationary-geometric}, $\Pr[X_{i+1} =k+1 | X_i = k] = 1/2$ and $\Pr[X_{i+1} =1 | X_i = k] = 1/2$. Assuming $\pi_i$ is the stationary distribution for $X_i$ then we can write $\pi_1 = 1/2 \sum_{j=1}^{\infty} \pi_j = 1/2$ and recursively for each $i$, $\pi_i = 1/2 \pi_{i-1} = (1/2)^i$.
\end{proof}

The following lemma can be verified using a coupling argument with a chain $X$ starting at $1$ and a chain $Y$ starting at the stationary distribution. We can estimate 
\todo{DD: use mathrm for non-variable text}
$t_\mathrm{mix}(\epsilon)$ by estimating $\Pr_Z{(X_T \neq Y_T)}$. 

\cite[find citation]{?}

Let $X_n$ and $Y_n$ be Markov chains over $(S, P)$ with initial distributions $\mu$ and $v$, respectively. Let $Z_n = (X_n, Y_n)$ be a coupling of $X_n$ and $Y_n$.
Then $d_V (\mu_n, v_n) \leq \Pr_Z(X_n \neq Y_n)$.

If $\Pr_Z(X_T \neq Y_T | X_0 = x, Y_0 \text{ distributed according to } \pi) \leq \epsilon$ then $t_{mix}(\epsilon) < T$.

\begin{lemma}[Section 5.3.5, \cite{levin2017markov}]\label{lem:sg-mixing-time}
$t_{mix}(\epsilon) \leq \ceil{\log(\frac{1}{\epsilon})}$; 
\end{lemma}

\begin{corollary}
by Lemma~\ref{lem:sg-mixing-time}, $t_{mix}(\frac{1}{n}) \leq \ceil{\log(n)}$, thus after $\log n$ steps of the $\SG$'s Markov chain, for all $i$ the actual probabilities are not far from the stationary probabilities:
$|\Pr(\SG = i) - \pi_i| \leq 1/n$
\end{corollary}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Using stationary distribution:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{lemma}\label{lem:reset-count-down-stationary}
% \cite[Section 5.1]{alistarh17detection} stationary distribution:
% \end{lemma}


% \begin{proof}
% \todoi{Maybe replace all $p_{i, j}$ with $\Pr{\signalArray[i] = j}$.}
% Let $p_{i, j}$ be the probability that the agent has value $j$ in the $i^{th}$ index of its $\signalArray$. Recall that $M_i$ denote the maximum value for signal $i$, then $p_{i, M_i} = 1/2^i$ (by equation 9~\ref{?}). We define $p_{i, \geq j} = p_{i, j} + p_{i, j+1} + \ldots + p_{i, M_i}$ the probability that an agent has a value greater than $j$ for signal $i$. We want to calculate $p_{i, \geq 1}$.  

% Note that for the analysis of our protocol, we don't need to know the exact counts of the agents who have value $j$ for $0 < j < M_i$ for each signal $i$; instead, we show that the agents' values remains above $0$ for $\log \log n < i < 1/2 \log n$. 

% % To do so, we analyze the stationary probability for $p_{i,\geq 1}$.
% Fix an agent $u$, an interaction $d \in \N$, and let $1< j < M_i$.
% Then %agent $u$ has a value greater than or equal to  for signal $i$ if and only if:
% $u.\signalArray[i]_{d} \geq j$ if and only if


% 1) $u.\signalArray[i]_{d-1} \geq j$
% % It had value $j$ before 
% and $a$ is not selected in the $d$-th interaction.
% ??? with probability $1-\frac{2}{n}$.

% 2) For the $d$-th interaction, the scheduler selects agents $u$ 
% %with probability $2/n$ 
%  and $v$ and $\max(u.\signalArray[i]_{d-1}, v.\signalArray[i]_{d-1}) > j$.
% %or $v$ have a value $> j$ for signal $i$.

% Thus we have the recurrence
% \begin{align*}
% p_{i, \geq j} 
% &= \left(1-\frac{2}{n}\right) \cdot p_{i, \geq j } 
% + \frac{2}{n} \cdot \left[1- (1- p_{i, \geq j+1})^2 \right]
% \end{align*}
% Specifically for $j = 1$ we have:
% \begin{align*}
% p_{i, \geq 1} 
% &= \left(1-\frac{2}{n}\right) \cdot p_{i, \geq 1} 
% + \frac{2}{n} \cdot \left[1- (1- p_{i, \geq 2})^2 \right]\\
% \end{align*}


% we can use $p_{i, \geq M_i} = 1/2^i$ to solve the above recursion which results to the following formula:
% % Hence, to compute the stationary probability we can use the following equations: 

% % And for the maximum value of each signal, we know that $p_{i, \geq M_i} \geq L_i/n$. We can Solving the closed form of the above recursion results in to a formula similar to~\cite{alistarh17detection}:
% \begin{equation*}
% p_{i, \geq 1} = 1- \left(1-\frac{1}{2^i} \right) ^{2^{M_i}}    
% \end{equation*}
% % Recall that in the above formula  $L_i/n$ is the minimum fraction of agents that hold $\group = i$ (Lemma~\ref{lem:independent-sg-fraction-bounds}) and $M_i$ is the maximum value defined in Protocol~\ref{protocol:reset-count-down} for each signal $i$.
% \end{proof}

